Cross-Chain Payment Protocols with Success Guarantees

In this paper, we consider the problem of cross-chain payment whereby customers of different escrows -- implemented by a bank or a blockchain smart contract -- successfully transfer digital assets without trusting each other. Prior to this work, cross-chain payment problems did not require this success or any form of progress. We introduce a new specification formalism called Asynchronous Networks of Timed Automata (ANTA) to formalise such protocols. We present the first cross-chain payment protocol that ensures termination in a bounded amount of time and works correctly in the presence of clock skew. We then demonstrate that it is impossible to solve this problem without assuming synchrony, in the sense that each message is guaranteed to arrive within a known amount of time. We also offer a protocol that solves an eventually terminating variant of this cross-chain payment problem without synchrony, and even in the presence of Byzantine failures.

==> ABC.tex <==
\expandafter\ifx\csname graph\endcsname\relax
   \csname newbox\expandafter\endcsname\csname graph\endcsname
\fi
\ifx\graphtemp\undefined
  \csname newdimen\endcsname\graphtemp
\fi
\expandafter\setbox\csname graph\endcsname
 =\vtop{\vskip 0pt\hbox{%
\pdfliteral{
q [] 0 d 1 J 1 j
0.576 w
1.008 w
54 -18 m
54 -27.941125 41.911688 -36 27 -36 c
12.088312 -36 0 -27.941125 0 -18 c
0 -8.058875 12.088312 0 27 0 c
41.911688 0 54 -8.058875 54 -18 c
S
Q
}%
    \graphtemp=.5ex
    \advance\graphtemp by 0.250in
    \rlap{\kern 0.375in\lower\graphtemp\hbox to 0pt{\hss Alice\hss}}%
\pdfliteral{
q [] 0 d 1 J 1 j
1.008 w
0.576 w
113.4 -64.368 m
167.4 -64.368 l
167.4 -28.368 l
113.4 -28.368 l
113.4 -64.368 l
S
Q
}%
    \graphtemp=.5ex
    \advance\graphtemp by 0.644in
    \rlap{\kern 1.950in\lower\graphtemp\hbox to 0pt{\hss Escrow 0\hss}}%
\pdfliteral{
q [] 0 d 1 J 1 j
0.576 w
0.072 w
q 0 g
107.28 -33.552 m
113.4 -38.232 l
105.696 -38.952 l
107.28 -33.552 l
B Q
1.512 w
54 -20.808 m
106.488 -36.216 l
S
0.576 w
54 -74.664 m
54 -84.605125 41.911688 -92.664 27 -92.664 c
12.088312 -92.664 0 -84.605125 0 -74.664 c
0 -64.722875 12.088312 -56.664 27 -56.664 c
41.911688 -56.664 54 -64.722875 54 -74.664 c
S
Q
}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.037in
    \rlap{\kern 0.375in\lower\graphtemp\hbox to 0pt{\hss Chloe\hss}}%
\pdfliteral{
q [] 0 d 1 J 1 j
0.576 w
0.072 w
q 0 g
105.696 -53.712 m
113.4 -54.432 l
107.28 -59.184 l
105.696 -53.712 l
B Q
1.512 w
54 -71.856 m
106.488 -56.448 l
S
0.576 w
113.4 -121.032 m
167.4 -121.032 l
167.4 -85.032 l
113.4 -85.032 l
113.4 -121.032 l
S
Q
}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.431in
    \rlap{\kern 1.950in\lower\graphtemp\hbox to 0pt{\hss Escrow 1\hss}}%
\pdfliteral{
q [] 0 d 1 J 1 j
0.576 w
0.072 w
q 0 g
107.28 -90.216 m
113.4 -94.968 l
105.696 -95.688 l
107.28 -90.216 l
B Q
1.512 w
54 -77.544 m
106.488 -92.952 l
S
0.576 w
54 -131.4 m
54 -141.341125 41.911688 -149.4 27 -149.4 c
12.088312 -149.4 0 -141.341125 0 -131.4 c
0 -121.458875 12.088312 -113.4 27 -113.4 c
41.911688 -113.4 54 -121.458875 54 -131.4 c
S
Q
}%
    \graphtemp=.5ex
    \advance\graphtemp by 1.825in
    \rlap{\kern 0.375in\lower\graphtemp\hbox to 0pt{\hss Bob\hss}}%
\pdfliteral{
q [] 0 d 1 J 1 j
0.576 w
0.072 w
q 0 g
105.696 -110.448 m
113.4 -111.096 l
107.28 -115.848 l
105.696 -110.448 l
B Q
1.512 w
54 -128.52 m
106.488 -113.112 l
S
Q
}%
    \hbox{\vrule depth2.075in width0pt height 0pt}%
    \kern 2.325in
  }%
}%

